Maximal Information Leakage based Privacy Preserving Data Disclosure Mechanisms

It is often necessary to disclose training data to the public domain, while protecting privacy of certain sensitive labels. We use information theoretic measures to develop such privacy preserving data disclosure mechanisms. Our mechanism involves perturbing the data vectors in a manner that strikes a balance in the privacy-utility trade-off. We use maximal information leakage between the output data vector and the confidential label as our privacy metric. We first study the theoretical Bernoulli-Gaussian model and study the privacy-utility trade-off when only the mean of the Gaussian distributions can be perturbed. We show that the optimal solution is the same as the case when the utility is measured using probability of error at the adversary. We then consider an application of this framework to a data driven setting and provide an empirical approximation to the Sibson mutual information. By performing experiments on the MNIST and FERG data-sets, we show that our proposed framework achieves equivalent or better privacy than previous methods based on mutual information.

==> Sections/ClassicDetectionGaussianCase.tex <==
\section{Affine transformation of Gaussian data}
\subsection{Gaussian data setup}
In this section, we consider the same theoretical data setting as \cite{CGAPpaper} where both the privatizer and and the adversary have access to the joint distributions of the public variable $X$ and the private variable $C$ as $P(X,C)$. The problem of interest is to optimize a privacy mapping on the transformed data for the privatizer, subject to a distortion constraint on the transformation. The parameters of the optimization are $\beta_0, \beta_1$, and the optimal values are the result of minimizing the adversary's accuracy $Pr(\hat{C} = C)$. The adversary knows the distribution and therefore only needs to compute its guess via the MAP decision rule.
%You have not defined what $C$ and $X$.
The data distribution for $X$ follows a mixture of two Gaussians:
\begin{multline}\label{eq:1}
    p(X|C=0) \sim \mathcal{N}(\mu_0, \sigma^2), \quad p(X|C=1) \sim \mathcal{N}(\mu_1, \sigma^2)
\end{multline}
with conditional probabilities 
\begin{flalign}\label{eq:2}
    P(C=0) = \tilde{p}, \quad P(C=1) = 1-\tilde{p}
\end{flalign}
\subsection{Affine transformation}
W.L.O.G. we may let $\mu_0 \le \mu_1$. We let the Gaussian distributions have equal covariance for tractability purposes, and define the following data-dependent affine transformation of the data: $Z = X + (1 - C)\beta_0 + C\beta_1$. This transformation is dependent on the parameters $\beta_0, \beta_1$, and can be seen in Figure \ref{fig:Affine transform}.
\begin{flalign}\label{eq:3}
    p(Z|C=0) \sim \mathcal{N}(\mu_0 + \beta_0, \sigma^2) = \mathcal{N}(\mu_0^{'}, \sigma^2), \\
    p(Z|C=1) \sim \mathcal{N}(\mu_1 - \beta_1, \sigma^2) = \mathcal{N}(\mu_1^{'}, \sigma^2) \\
    \beta_0, \beta_1 \ge 0 \\
    \mu_0^{'} \le \mu_1^{'} \label{eq:6}
\end{flalign}

\begin{figure}[!h]
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt
\resizebox {\columnwidth} {!} {
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,209); %set diagram left start at 0, and has height of 209

%Shape: Axis 2D [id:dp5262504800310911] 
\draw  (17,125) -- (435,125)(226.72,29) -- (226.72,146) (428,120) -- (435,125) -- (428,130) (221.72,36) -- (226.72,29) -- (231.72,36)  ;
%Curve Lines [id:da24078169182249698] 
\draw [color={rgb, 255:red, 134; green, 206; blue, 63 }  ,draw opacity=1 ]   (273,118) .. controls (314,110) and (330,31) .. (358,63) .. controls (386,95) and (389,115) .. (419,120) ;


%Curve Lines [id:da5294539646661326] 
\draw [color={rgb, 255:red, 17; green, 22; blue, 231 }  ,draw opacity=1 ]   (34,116) .. controls (75,108) and (91,29) .. (119,61) .. controls (147,93) and (151,115) .. (179,116) ;


%Curve Lines [id:da9247585206729886] 
\draw [color={rgb, 255:red, 17; green, 22; blue, 231 }  ,draw opacity=1 ]   (102,116) .. controls (143,108) and (159,29) .. (187,61) .. controls (215,93) and (219,115) .. (247,116) ;


%Curve Lines [id:da204757087678484] 
\draw [color={rgb, 255:red, 134; green, 206; blue, 63 }  ,draw opacity=1 ]   (228,117) .. controls (269,109) and (285,30) .. (313,62) .. controls (341,94) and (344,114) .. (374,119) ;


%Straight Lines [id:da8771464093361935] 
\draw    (107,53) -- (169,52.03) ;
\draw [shift={(171,52)}, rotate = 539.1] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8001950290884339] 
\draw    (345,54) -- (304,54) ;
\draw [shift={(302,54)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (99,142) node   {$P( X|C=0)$};
% Text Node
\draw (359,141) node   {$P( X|C=1)$};
% Text Node
\draw (138,41) node   {$\beta _{0}$};
% Text Node
\draw (324,41) node   {$\beta _{1}$};
% Text Node
\draw (439,109) node   {$x$};
% Text Node
\draw (229,14) node   {$P( x)$};

\end{tikzpicture}
}
\caption{Binary Gaussian data and transformation vectors}
\label{fig:Affine transform}
\end{figure}

%Draw a diagram for the transform
\subsection{Optimization problem and solutions}
Under affine transformations the optimized Z data distribution is intuitively moving the means of the distributions closer to each other, and the adversary's MAP rule assumes that the shifted means still satisfy $\mu_0^{'} \le \mu_1^{'}$. The parameters are constrained to be within the set $\mathcal{D}$ to adhere to a distortion constraint:
\begin{flalign}
    \mathcal{D} = \{(\beta_0, \beta_1)|(1-\tilde{p})\beta_0^2 + \tilde{p}\beta_1^2 \le D , \beta_0 \ge 0, \beta_1 \ge 0\} \label{eq:affine D definition}
\end{flalign}
Under the aforementioned circumstances the optimization problem is 
\begin{flalign}
&\max_{(\beta_0, \beta_1) \in \mathcal{D}} \frac{\mu_0^{'} - \mu_1^{'}}{2\sigma} \label{eq:initial optimization problem def}
\end{flalign}
The solution to this optimization problem is 
\begin{equation}
    \beta_0^* = \sqrt{\frac{\tilde{p}}{1 - \tilde{p}} D}, \qquad \beta_1^* = \sqrt{\frac{1 - \tilde{p}}{\tilde{p}} D} \label{eq:affine solution 1}
\end{equation}
if $D$ satisfies
\begin{flalign}
    D \le \Big(\frac{\mu_1 - \mu_0}{\sqrt{\frac{\tilde{p}}{1 - \tilde{p}}} + \sqrt{\frac{1 - \tilde{p}}{\tilde{p}}}}\Big)^2 \label{eq:affine solution condition}
\end{flalign}
and
\begin{flalign}
    \beta_0^* = (\mu_1 - \mu_0)(1 - \tilde{p}), \qquad
    \beta_1^* = (\mu_1 - \mu_0)\tilde{p} \label{eq:affine solution 2}
\end{flalign}
Refer to Appendix 1 Section A for detailed solutions.

In the following subsections, we will refer to the previous work \cite{CGAPpaper} using MAP accuracy as the metric which results in equation (\ref{eq:affine solution 1}) as their solution, maximal information leakage, and Sibson mutual information as privacy metrics in the optimization. All of these privacy metrics allow us to recover the same optimization problem and hence the same solution in equation (\ref{eq:affine solution 1}, \ref{eq:affine solution 2}).

\subsection{MAP accuracy as a metric}
In this section we consider the optimization for the same transformation as above with the MAP adversary's accuracy as the privacy metric, as prior work\cite{CGAPpaper} has done. Their theorem recovers the solution in equation (\ref{eq:affine solution 1}) but not the solution in equation (\ref{eq:affine solution 2}) with condition (\ref{eq:affine solution condition}). The distortion constraint is directly over the parameters of the distribution, and is used to illustrate a privacy-utility trade-off where the utility is characterized by the distortion budget and the privacy is the adversary's accuracy. This leads to a characterization of the adversary's accuracy in terms of the distortion constraint with the following theorem:
\begin{theorem}
Under the binary Gaussian data scenario with affine transformations of the data described in the set of equations and inequalities \ref{eq:1} - \ref{eq:6} over the set $\mathcal{D}$, the adversary's accuracy after solving the optimization for the optimal parameters $(\beta_0^*, \beta_1^*)$
\begin{flalign}
    (\beta_0^*, \beta_1^*) = \argmin_{(\beta_0, \beta_1) \in \mathcal{D}} Pr(\hat{C} = C)
\end{flalign} is
\begin{flalign}
    \tilde{p}Q\big(\frac{\sigma}{\mu_0^{'} - \mu_1^{'}}\log(\frac{1 - \tilde{p}}{\tilde{p}}) - \frac{\mu_0^{'} - \mu_1^{'}}{2 \sigma}\big) + \\
    (1 - \tilde{p})Q\big(- \frac{\sigma}{\mu_0^{'} - \mu_1^{'}}\log(\frac{1 - \tilde{p}}{\tilde{p}}) - \frac{\mu_0^{'} - \mu_1^{'}}{2 \sigma}\big) \nonumber%, \mu_0^{'} \le \mu_1^{'}
    \label{eq: MAP accuracy expression}
\end{flalign}
and $(\beta_0^*, \beta_1^*)$ are given by the solution to the optimization in equation (\ref{eq:initial optimization problem def})
\begin{equation}
    \beta_0^* = \sqrt{\frac{\tilde{p}}{1 - \tilde{p}} D}, \qquad \beta_1^* = \sqrt{\frac{1 - \tilde{p}}{\tilde{p}} D}
\end{equation}
if $D$ satisfies
\begin{flalign}
    D \le \Big(\frac{\mu_1 - \mu_0}{\sqrt{\frac{\tilde{p}}{1 - \tilde{p}}} + \sqrt{\frac{1 - \tilde{p}}{\tilde{p}}}}\Big)^2
\end{flalign}
and
\begin{flalign}
    \beta_0^* = (\mu_1 - \mu_0)(1 - \tilde{p}), \qquad
    \beta_1^* = (\mu_1 - \mu_0)\tilde{p}
\end{flalign}
otherwise.\\
\textbf{Proof:} Refer to Appendix 1 Section B.
\end{theorem}
Note that the above solution is under the assumption that $\mu_0 \le \mu_1$ and $\mu_0^{'} \le \mu_1^{'}$, since the MAP decision rule would be reversed if the means are shifted over each other. In \cite{CGAPpaper}, their game theoretic solutions are the same as ours for optimization over the MAP adversary accuracy in equation (\ref{eq:affine solution 1}), but we specify a constraint on the distortion budget $D$ (equation \ref{eq:affine solution condition}) that gives another solution (equation \ref{eq:affine solution 2}) when the condition is not satisfied.

\subsection{Maximal Information Leakage as a metric}
Now we propose using maximal information leakage as an optimization metric, and investigate the induced optimization problem based on the same synthetic data distributions and affine transformation as the previous section.
The maximal information leakage is defined as:
\begin{equation}
    I_{\infty}(C; Z) = \log(\displaystyle\sum_z \max_c p_{Z|C}(z|c))
\end{equation}
The optimization solution is now:
\begin{flalign}
    (\beta_0^*, \beta_1^*) = \argmin_{(\beta_0, \beta_1) \in \mathcal{D}} I_{\infty}(C; Z)
\end{flalign}
The following theorem equates the optimization problem to the optimization in equation (\ref{eq:initial optimization problem def}), and characterizes the solutions of the optimization.
\begin{theorem}
Under binary mixture of Gaussians data described in equations \ref{eq:1} - \ref{eq:6} over the set $\mathcal{D}$, assuming $\mu_0^{'} < \mu_1^{'}$, the solution to minimization of maximal information leakage is equal to
\begin{flalign}
&(\beta_0^*, \beta_1^*) = \argmin_{(\beta_0, \beta_1) \in \mathcal{D}} \log\big(2 Q(\frac{\mu_0^{'} - \mu_1^{'}}{2\sigma})\big) = \\
&\argmax_{(\beta_0, \beta_1) \in \mathcal{D}} \big(\frac{\mu_0^{'} - \mu_1^{'}}{2\sigma}\big)
\end{flalign}
and the solutions $\beta_0^*, \beta_1^*$ are given by equations (\ref{eq:affine solution 1}, \ref{eq:affine solution 2}).\\
\textbf{Proof:} Under the mixture of Gaussians distribution and assuming that $\mu_0^{'} < \mu_1^{'}$, we have:
\begin{equation}
    I_{\infty}(C; Z) = \log \Big(\displaystyle\int_{-\infty}^{z_0} p_{Z|C=0} + \displaystyle\int_{z_0}^{\infty} p_{Z|C=1}\Big)
\end{equation}
The intersection point can be found in this scenario as 
\begin{equation}
    z_0 = \frac{\mu_1^{'2} - \mu_0^{'2}}{2(\mu_1^{'} - \mu_0^{'})} = \frac{\mu_1^{'} + \mu_0^{'}}{2}
\end{equation}
Hence solving the optimization objective of minimizing the maximal information leakage subject to a distortion constraint is equivalent to:
\begin{flalign}
&\argmin_{(\beta_0, \beta_1) \in \mathcal{D}} \log\Big((1-Q(\frac{z_0 - \mu_0^{'}}{\sigma})) + Q(\frac{z_0 - \mu_1^{'}}{\sigma})\Big) \\
&= \argmin_{(\beta_0, \beta_1) \in \mathcal{D}} \log\Big((1-Q(\frac{\mu_1^{'} - \mu_0^{'}}{2\sigma})) + Q(\frac{\mu_0^{'} - \mu_1^{'}}{2\sigma})\Big) \\
&= \argmin_{(\beta_0, \beta_1) \in \mathcal{D}} \log\Big(2 Q(\frac{\mu_0^{'} - \mu_1^{'}}{2\sigma})\Big) = \argmax_{(\beta_0, \beta_1) \in \mathcal{D}} \frac{\mu_0^{'} - \mu_1^{'}}{2\sigma}
%&= \argmax_{(\beta_0, \beta_1) \in \mathcal{D}} \mu_0 + \beta_0 - (\mu_1 - \beta_1) = \argmax_{(\beta_0, \beta_1) \in \mathcal{D}} \beta_0 + \beta_1
\end{flalign}
The optimization is the same as the one proposed in equation (\ref{eq:initial optimization problem def}), subject to the constraints specified in equation \ref{eq:6} and \ref{eq:affine D definition}, and yields the same results for $\beta_0^*, \beta_1^*$
\qedsymbol
\end{theorem}
Therefore when optimizing the maximal information leakage for the defined data distribution and transformation, it is equivalent to minimizing an adversary's theoretical performance, and both reduce to minimizing the distance between the means of the transformed Gaussian distributions.




==> Sections/DataDrivenApproach.tex <==
\section{Data driven approach for maximal information leakage}

\begin {figure}
\centering
\resizebox {0.7\columnwidth} {!} {
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt     

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Flowchart: Connector [id:dp8875211609125826] 
\draw   (114,76) .. controls (114,56.67) and (129.67,41) .. (149,41) .. controls (168.33,41) and (184,56.67) .. (184,76) .. controls (184,95.33) and (168.33,111) .. (149,111) .. controls (129.67,111) and (114,95.33) .. (114,76) -- cycle ;
%Flowchart: Connector [id:dp6992743099510927] 
\draw   (117,218) .. controls (117,198.67) and (132.67,183) .. (152,183) .. controls (171.33,183) and (187,198.67) .. (187,218) .. controls (187,237.33) and (171.33,253) .. (152,253) .. controls (132.67,253) and (117,237.33) .. (117,218) -- cycle ;
%Flowchart: Connector [id:dp2970622183597329] 
\draw   (280,148) .. controls (280,128.67) and (295.67,113) .. (315,113) .. controls (334.33,113) and (350,128.67) .. (350,148) .. controls (350,167.33) and (334.33,183) .. (315,183) .. controls (295.67,183) and (280,167.33) .. (280,148) -- cycle ;
%Flowchart: Connector [id:dp59894773071282] 
\draw   (434,81) .. controls (434,61.67) and (449.67,46) .. (469,46) .. controls (488.33,46) and (504,61.67) .. (504,81) .. controls (504,100.33) and (488.33,116) .. (469,116) .. controls (449.67,116) and (434,100.33) .. (434,81) -- cycle ;
%Flowchart: Connector [id:dp5686527484563878] 
\draw   (437,225) .. controls (437,205.67) and (452.67,190) .. (472,190) .. controls (491.33,190) and (507,205.67) .. (507,225) .. controls (507,244.33) and (491.33,260) .. (472,260) .. controls (452.67,260) and (437,244.33) .. (437,225) -- cycle ;
%Straight Lines [id:da2485311461924331] 
\draw    (184,76) -- (278.4,146.8) ;
\draw [shift={(280,148)}, rotate = 216.87] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da10611281392752192] 
\draw    (187,218) -- (278.4,149.2) ;
\draw [shift={(280,148)}, rotate = 503.03] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8220237777560772] 
\draw    (350,148) -- (432.44,82.25) ;
\draw [shift={(434,81)}, rotate = 501.42] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da40154819928185914] 
\draw    (350,148) -- (435.5,223.67) ;
\draw [shift={(437,225)}, rotate = 221.51] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (149,75) node [scale=1.44] [align=left] {$\displaystyle X$};
% Text Node
\draw (152,218) node [scale=1.44] [align=left] {$\displaystyle C$};
% Text Node
\draw (315,147) node [scale=1.44] [align=left] {$\displaystyle Z$};
% Text Node
\draw (468,80) node [scale=1.44] [align=left] {$\displaystyle \hat{X}$};
% Text Node
\draw (470,222) node [scale=1.44] [align=left] {$\displaystyle \hat{C}$};
% Text Node
\draw (372,210.5) node  [align=left] {Adversary $\displaystyle g$};
% Text Node
\draw (300.5,79.5) node  [align=left] {Privatizer $\displaystyle f$};


\end{tikzpicture}

}
\caption{Graph representation of the adversarial privatization model}
\label{fig: graph representation}
\end{figure}

For a dataset consisting of N pairs of $(X, C)$ in $\{(X^{(n)}, C^{(n)})\}_{n=1}^N$, the problem is to find some (randomized) mapping $(X, C) \rightarrow Z$ such that the privatized representation leaks as little information as possible with regards to the private variable. The data $X$ is assumed to be continuous, and the private variable $C$ is a discrete variable correlated with $X$ with $G$ different possible values, often the class which $X$ belongs to. \iffalse Due to the fact that maximal information leakage is not differentiable with respect to parameters of the transformation $Z \sim \mathcal{N}(f_{\mu}(x, c), f_{\Sigma}(x,c))$, we use the Sibson mutual information of order 20 for our experiments. \fi We use Sibson mutual information of order 20 in our experiments. This approximation is sufficiently close to the Sibson mutual information at order $\infty$ and do not result in numerical over/underflow during the optimization.

In order to learn the mapping, we make use of neural networks to parameterize the adversary and privatizer, in an auto-encoding model shown in Fig \ref{fig: graph representation}. The adversary is trained to make inferences, and the privatizer is trained to minimize the privacy metric and adhere to a distortion budget. For synthetic data, we also conduct experiments with (noisy) affine encoders instead, but the adversary is still represented by a neural network. When we are using neural networks to parameterize the encoder in experiments, we measure distortion as the average reconstruction error by default
\begin{flalign}
&\mathop{{}\mathbb{E}}_x[d(X, \hat{X})] = \frac{1}{N}\displaystyle\sum_n^N d(X^{(n)}, \hat{X}^{(n)}) \le D\\
&d(X,\hat{X}) = ||X - \hat{X}||_2^2 \label{eq: L2distortion}
\end{flalign}
When using (noisy) affine transformations in the encoder, we measure the distortion as 
\begin{flalign}
    (1-\tilde{p})\beta_0^2 + \tilde{p}\beta_1^2 \le D
\end{flalign}
or 
\begin{flalign}
    (1 - \tilde{p})\beta_0^2 + \tilde{p}\beta_1^2 + \gamma^2 \le D
\end{flalign}
. For experiments with the synthetic Gaussian data, in the case of an affine transformation, measuring the expected L2 distance from the reconstruction $\hat{X} = Z$ to the original $X$ is equivalent to measuring $(1-\tilde{p})\beta_0^T \beta_0 + \tilde{p}\beta_1^T \beta_1$ up to a scaling factor in $D$. However, for neural networks learning non-linear mappings to the private representation, it is more appropriate to measure the distortion in terms of the average reconstruction error $\mathop{{}\mathbb{E}}_x[d(X, \hat{X})]$.

The privatizer $f(x, c) = (f_{\mu}(x,c), f_{\Sigma}(x,c))$ outputs the parameters of the conditional $Z$ distribution $P(Z|X,C)$, and $S$ samples of $Z$ are used as inputs to the adversary. The adversary $g(z)$ outputs predictions for $C$ in the vector $P(\hat{C}|Z)$ and the reconstruction in the vector $\hat{X}$ given the average over the $S$ samples of $Z$.

In the dataset we have $N$ pairs of data, and throughout training we assume the adversary is trained and generates posterior probability vectors that can classify the private labels with high accuracy. The posterior probability is used as part of the empirical loss function discussed below. Both the adversary $f$ and the privatizer $g$ are neural networks each parameterized by \begin{math}
\theta_p
\end{math} and \begin{math}
\theta_a
\end{math}.

\iffalse
, and the adversary's objective is to minimize its loss function which is the cross-entropy over the $G$ classes
\begin{flalign}
&L_{CE}(\theta_a) = \sum_n^N \sum_c^G \mathbbm{1}(C^{(n)}=c)(-\log(P(\hat{C}^{(n)}=c|Z^{(n)};\theta_a)))
\end{flalign}
whereas the privatizer's objective is to minimize the empirical Sibson mutual information. 
\begin{flalign}
&L_{p}(\theta_p) = I_{\alpha}(C;Z| \theta_a)
\end{flalign}
\fi

The goal in the data-driven approach is to learn a mapping for data pairs such that the Sibson mutual information is low, subject to a distortion constraint.
%\begin{flalign*}
%&\theta_a^* = \argmin_{\theta_a} \mathop{{}\mathbb{E}}_{X,C}[L_{CE}(P(\hat{C}|Z), C)], s.t. \quad \mathop{{}\mathbb{E}}[d(X, \hat{X})] \le D\\
%&\theta_p^* = \argmin_{\theta_p} \mathop{{}\mathbb{E}}_{X,C}[I_{\alpha}(C; Z|\theta_a^*)], s.t. \quad \mathop{{}\mathbb{E}}[d(X, \hat{X})] \le D
%\end{flalign*}
The optimal parameters for $\theta_p, \theta_a$ are found through an iterative alternating training algorithm to keep the adversary optimal for each iteration of optimization for the privatizer over the empirical approximation of the Sibson mutual information, which are further discussed.

\subsection{Empirical loss}
In this section we will discuss our approximation of the maximal information leakage as a metric for a data-driven privatization model, and compare it with conventional mutual information. We have access to the MAP adversary's guess of the $\hat{C}$ variable after the observation of $Z$, and along with a predetermined prior probability of $C$ which the MAP adversary also has access to, we may approximate the Sibson mutual information by using the empirical estimate of the posterior on $\hat{C}$:
\small
\begin{flalign}
&I_{\alpha}(C;Z) = \frac{\alpha}{\alpha-1}\log(\displaystyle\int_z (\displaystyle\sum_c^G P_{Z|C}^{\alpha}(z|c)P_C(c))^{1/\alpha} dz) \\
&= \frac{\alpha}{\alpha-1}\log(\displaystyle\int_z (\displaystyle\sum_c^G P_{C|Z}^{\alpha}(c|z)P_Z^{\alpha}(z)P_C(c)/P_C^{\alpha}(c))^{1/\alpha} dz) \\
&= \frac{\alpha}{\alpha-1}\log(\displaystyle\int_z (\displaystyle\sum_c^G P_{C|Z}^{\alpha}(c|z) P_C^{1 - \alpha}(c))^{1/\alpha} P_Z(z) dz) \\
&= \frac{\alpha}{\alpha-1}\log\Big(\displaystyle\int_z \big(\displaystyle\sum_c^G P_{C|Z}^{\alpha}(c|z) P_C^{1 - \alpha}(c)\big)^{1/\alpha} *\\
&\quad\displaystyle\int_x P_{Z|X}(z|x) P_X(x) dxdz\Big) \nonumber\\
&\approx \frac{\alpha}{\alpha-1}\log(\displaystyle\sum_n^N \frac{1}{N} \displaystyle\int_z P_{Z|X}(z|x_n)\\
&(\displaystyle\sum_c^G P_{C|Z}^{\alpha}(c_n|z)  P_C^{1 - \alpha}(c_n))^{1/\alpha} dz)  \nonumber\\
&\approx \frac{\alpha}{\alpha-1}\log(\displaystyle\sum_n^N \frac{1}{N}(\displaystyle\sum_i^S \frac{1}{S}(\displaystyle\sum_c^G P_{C|Z}^{\alpha}(c_n|z_{i,n})P_C^{1-\alpha}(c_n))^{1/\alpha})) \\
&\approx \frac{\alpha}{\alpha-1}\log(\displaystyle\sum_n^N \frac{1}{N}(\displaystyle\sum_i^S \frac{1}{S}(\displaystyle\sum_c^G P_{\hat{C}|Z}^{\alpha}(c_n|z_{i,n})P_C^{1-\alpha}(c_n))^{1/\alpha})) \\
&= \frac{\alpha}{\alpha-1}\log(\displaystyle\sum_n^N \frac{1}{N}(\displaystyle\sum_i^S \frac{1}{S}(\displaystyle\sum_c^G (\frac{P_{\hat{C}|Z}(c_n|z_{i,n})}{P_C(c_n)})^{\alpha}P_C(c_n))^{1/\alpha})) \\
&= \frac{\alpha}{\alpha-1}\log(\displaystyle\sum_n^N \frac{1}{N}(\displaystyle\sum_i^S \frac{1}{S}\mathbb{E}_{C}[ (\frac{P_{\hat{C}|Z}(c_n|z_{i,n})}{P_C(c_n)})^{\alpha}]^{1/\alpha}))
\label{eq: sibMI empirical}
\end{flalign}
\normalsize
Starting with the definition of the Sibson mutual information for a continuous $Z$ and discrete $C$ summed over its $G$ classes, we use Bayes' rule and then expand $P(Z)$ into $\sum_x P(Z|X)P(X)$. The summation over $P(X)$ can be approximated by the sum over the $N$ data points. Instead of integration over the support of $Z$, we average over samples of the conditional $Z$ distribution rather than compute due to the fact that outputting and summing over the classes $C$ is only available through the adversary, and the adversary takes discrete points of $Z$ as input. We use the estimated posterior on $C$ in the approximation because for every iteration of optimization over the privatizer, the adversary is trained and can produce an estimate $P(\hat{C}|Z)$ that is close to the true distribution.
In comparison, with mutual information, we have:
\begin{flalign}
&I(C;Z) = \displaystyle\int_z \displaystyle\sum_c^G P_{Z, C}(z, c) \log\Big(\frac{P_{C|Z}(c|z)}{P_C(c)}\Big)dz\\
&= \displaystyle\sum_n^N \frac{1}{N} \displaystyle\int_z \displaystyle\sum_c^G P_{C|Z}(c_n|z) P_{Z|X}(z|x_n) \log\Big(\frac{P_{C|Z}(c_n|z)}{P_C(c_n)}\Big)dz\\
&\approx \displaystyle\sum_n^N \frac{1}{N}\displaystyle\sum_i^S \frac{1}{S} \displaystyle\sum_c^G P_{C|Z}(c_n|z_{i,n}) \log\Big(\frac{P_{C|Z}(c_n|z_{i,n})}{P_C(c_n)} \Big)
\end{flalign}
The Sibson mutual information estimate allows us to design an adversarial model to minimize it when learning the privacy mapping. Our model consists of encoder and decoders parameterized by neural networks (represented in Fig 1), and the training procedure are discussed in the following section.

\subsection{Alternating training algorithm}
The encoder acts as a privatizer operating under the assumption that an optimal adversary is available, and optimizes to minimize the Sibson mutual information \begin{math}
I_{\alpha}(C;Z)
\end{math} subject to the same distortion budget $D$. They are each parameterized by \begin{math}
\theta_p
\end{math} and \begin{math}
\theta_a
\end{math} respectively. The models are trained for 2000 epochs for synthetic data, 400 epochs for MNIST data-set, and 400 for FERG data. Each epoch consists of a pass over all data points in the training set divided in mini-batches of size $M$ for a total of $N/M$ iterations, and the empirical Sibson mutual information/cross-entropy is computed below for each mini-batch. The adversary is trained with its objective $l$ as the cross-entropy loss for $k = 20$ iterations for each iteration of training for the privatizer. The objective functions for each component for each mini-batch of size $M$ at iteration $t$ are:
\begin{flalign}
&L_a(\theta_p^t, \theta_a^t, \rho_t) =  L_{CE}(P(\hat{C}_m|Z_m;\theta_a^t|\theta_p^t), C_m) \label{eq: minibatch L_a}\\
&+ \rho_t \max\Big\{0, \frac{1}{M} \displaystyle\sum_{m=1}^{M}d(\hat{x}_m, x_m) - D\Big\} \nonumber \\
&L_{CE}(P(\hat{C}_m|Z_m;\theta_a^t|\theta_p^t), C_m) = \\
&\frac{1}{M} \displaystyle \sum_{n=1}^{M}\sum_c^G \mathbbm{1}(C^{(n)}=c)[-\log(P(\hat{C}^{(n)}=c|Z^{(n)};\theta_a^t|\theta_p^t))]\\
&L_p(\theta_p^t, \theta_a^t, \rho_t) = I_{\alpha}(\hat{C}_m;Z_m | \theta_a^t) \label{eq: minibatch L_p}\\
&+ \rho_t \max\Big\{0, \frac{1}{M} \displaystyle\sum_{m=1}^{M}d(\hat{x}_m, x_m) - D\Big\} \nonumber\\
&I_{\alpha}(\hat{C}_m;Z_m | \theta_a^t, \theta_p^t) =\frac{\alpha}{\alpha-1} \cdot\\
&\log\Big(\displaystyle\sum_n^M \frac{1}{M}\big(\displaystyle\sum_i^S \frac{1}{S}(\displaystyle\sum_c^G (\frac{P_{\hat{C}|Z}(c_n|z_{i,n}; \theta_p^t|\theta_a^t)}{P_C(c_n)})^{\alpha}P_C(c_n))^{1/\alpha}\big)\Big)
\end{flalign}
The adversary's loss is dependent on the posterior estimate $P(\hat{C}|Z;\theta_a^t|\theta_p^t)$, conditioned on the privatizer network's generated representation of $Z$; the privatizer's loss depends on the posterior estimate $P(\hat{C}|Z;\theta_p^t|\theta_a^t)$, conditioned on the adversary network's prediction of $\hat{C}$. The empirical estimate of the Sibson mutual information is derived from equation (\ref{eq: sibMI empirical}) for a mini-batch of size $M$.
For synthetic data, the distortion measure is the distortion budget 
\begin{flalign}
d(\hat{x}_m, x_m) = (1-\tilde{p})\beta_0^2 + \tilde{p}\beta_1^2
\end{flalign} for an affine privatizer, and 
\begin{flalign}
d(\hat{x}_m, x_m) = (1 - \tilde{p})\beta_0^2 + \tilde{p}\beta_1^2 + \gamma^2
\end{flalign}
for a noisy affine privatizer instead of the L2 distance specified in equation (\ref{eq: L2distortion}), and the penalty coefficient \begin{math}
\rho_t
\end{math} increases with the number of iterations \begin{math}
t
\end{math}. 
The algorithm is given in Algorithm \ref{alg: alternating training algorithm}.
\begin{algorithm}
    \caption{Alternate training for privacy-preserving adversarial model}
    \label{alternatealgo}
    \begin{algorithmic}
    \REQUIRE $M, S, N, k, D, \{c_i\}, \{x_i\}$
    \ENSURE $\theta_p^{T}, \theta_a^{T}$
    \STATE $\theta_p^0 \leftarrow 0, \theta_a^0 \leftarrow 0, t = 0$
    \WHILE{$t \le T$}
    \STATE $\rho_t = \frac{1000t}{T}$
    \STATE $\theta_a^{t,0} \leftarrow \theta_a^t$
    \FOR{$(j = 0; j < k; j++)$}
    \STATE $\theta_a^{t,j+1} \leftarrow f_{Adam}(\nabla_{\theta_a}L_a(\theta_p^t, \theta_a^{t,j}, \rho_t))$
    \COMMENT{$f_{Adam}$ is the output from one update of the Adam optimizer on the adversary's loss component}
    \ENDFOR
    \STATE $\theta_a^{t+1} \leftarrow \theta_a^{t,k-1}$
    \STATE $\theta_p^{t+1} \leftarrow g_{Adam}(\nabla_{\theta_p}L_p(\theta_p^t, \theta_a^{t+1}, \rho_t))$
    \COMMENT{$g_{Adam}$ is the output from one update of the Adam optimizer on the privatizer's loss component}
    \STATE $t \leftarrow t + 1$
    \ENDWHILE
    \RETURN $\theta_p^{T}, \theta_a^{T}$
    \end{algorithmic}
    \label{alg: alternating training algorithm}
\end{algorithm}

The reason for iterating over the training of the adversary $k$ times for each iteration of the privatizer training is to ensure that the adversary is sufficiently trained, and produces the posterior probabilities of the private labels that are able to classify them well. The inner loop updates the parameters of the adversary network $k$ times according to the adversary loss $L_a$ to maintain a trained adversary for every time the privatizer's parameters are updated. Therefore the privatizer will operate under the assumption that a trained adversary is present, as specified in the design of this model. In practice we used $k=20$ for training for synthetic data and $k=10$ for MNIST and FERG data.

==> Sections/MaxMIUnequalCovar.tex <==
\subsection{Extensions to unequal covariances}
Extending this framework to mixture of Gaussians data with unequal means and covariances, we do not have an analytical expression while using the MAP adversary approach derived from detection theory, but under the maximal information leakage metric, we may derive another optimization problem. We consider two Gaussians:
\begin{align*}
    p(X|C=0) \sim \mathcal{N}(\mu_0, \Sigma_0), \quad p(X|C=1) \sim \mathcal{N}(\mu_1, \Sigma_1)
\end{align*}
with conditional probabilities
\begin{align*}
    P(C=0) = \tilde{p}, \quad P(C=1) = 1-\tilde{p}
\end{align*}
The transformation under consideration is:
\begin{align*}
    Z = X + \beta_0 (1-C) + \beta_1 C + \gamma_0 (1-C) N + \gamma_1 C N,\\
    N \sim \mathcal{N}(0,1)
\end{align*}The resulting data is then from this distribution
\begin{align*}
    p(Z|C=0) \sim \mathcal{N}(\mu_0+\beta_0, \Sigma_0 + \gamma_0 I \gamma_0^T)\\ p(Z|C=1) \sim \mathcal{N}(\mu_1+\beta_1, \Sigma_1 + \gamma_1 I \gamma_1^T)
\end{align*}
From the definition of maximal information in the previous section,
\begin{gather*}
    \displaystyle\max_C P_{Z|C} = p_{Z|C=0} \Leftrightarrow p_{Z|C=0} > p_{Z|C=1}\\
    \frac{1}{\sqrt{2 \pi \sigma_0^2}} \exp(- \frac{(z - \mu_0^{'})^2}{2 \sigma_0^2}) > \frac{1}{\sqrt{2 \pi \sigma_1^2}} \exp(- \frac{(z - \mu_1^{'})^2}{2 \sigma_1^2})\\
    (z - \frac{\mu_0^{'}\sigma_1^2 - \mu_1^{'}\sigma_0^2}{\sigma_0^2 - \sigma_1^2})^2 < \frac{2 \sigma_1^2 \sigma_0^2\log\frac{\sigma_1^2}{\sigma_0^2}}{\sigma_1^2 - \sigma_0^2} + \frac{\mu_1^{'2}\sigma_0^2 - \mu_0^{'2}\sigma_1^2}{\sigma_1^2 - \sigma_0^2} +\\
    (\frac{\mu_0^{'}\sigma_1^2 - \mu_1^{'}\sigma_0^2}{\sigma_0^2 - \sigma_1^2})^2
\end{gather*}
This admits two solutions $z_0$ and $z_1$, W.L.O.G we may assume that $\sigma_1^2 - \sigma_0^2 > 0$, then the maximum will choose $p_{Z|C=0}$ for the range $[z_0, z_1]$. Thus we have
\begin{gather*}
    I_\infty(C;Z) = \log (\displaystyle\int_{z_0}^{z_1}P_{Z|C=0} + \displaystyle\int_{-\infty}^{z_0}P_{Z|C=1} +\\
    \displaystyle\int_{z_1}^{\infty}P_{Z|C=1})
\end{gather*}
This leads to the optimization objective expressed in terms of the Q function and subject to a distortion constraint on the transformed $Z$, but is optimized over the parameters $\beta_0, \beta_1, \sigma_0, \sigma_1$.
\begin{gather*}
    \min \log((1 - Q(z_0 - \mu_1^{'})) + Q(z_1 - \mu_1^{'}) + \\
    (Q(z_0 - \mu_0^{'}) - Q(z_1 - \mu_0^{'})))\\
    s.t. \quad \mathbb{E}[d(z, x)] \le D
\end{gather*}

\subsection{Extension to multi-class mixture of Gaussians data}
Now we extend the previous data setup to multi-class mixture of Gaussians, with 3 classes distributed as 
\begin{align*}
    \mathcal{N}(\mu_0, \Sigma), \mathcal{N}(\mu_1, \Sigma), \mathcal{N}(\mu_2, \Sigma)
\end{align*}
with prior probabilities $\tilde{p}_0, \tilde{p}_1, 1-\tilde{p}_0-\tilde{p}_1$ respectively and restrict our affine transformations to $Z = X + \beta_0 \mathbbm{1}(C=0) + \beta_1 \mathbbm{1}(C=1) + \beta_2 \mathbbm{1}(C=2)$. Through this transformation, the resulting data follows the conditional distributions 
\begin{align*}
    P(Z|C=0) \sim \mathcal{N}(\mu_0+\beta_0, \Sigma), \\
    P(Z|C=1) \sim \mathcal{N}(\mu_1+\beta_1, \Sigma), \\
    P(Z|C=2) \sim \mathcal{N}(\mu_2+\beta_2, \Sigma)
\end{align*}
Following the same definition of the maximal information leakage, we have the following expression:
\begin{align*}
    I_{\infty}(C; Z) = \log(\displaystyle\int_z \max_C p_{(Z|C)}) = \\
    \log(\displaystyle\int_{-\infty}^{z_0} p_{(Z|C=0)} + \displaystyle\int_{z_0}^{z_1} p_{(Z|C=1)} + \displaystyle\int_{z_1}^{\infty} p_{(Z|C=2)})
\end{align*}
W.L.O.G we may order the transformed Gaussians in the order $\mu_0^{'} \le \mu_1^{'} \le \mu_2^{'}$, then for each term we have $z_0 = \frac{\mu_0^{'} + \mu_1^{'}}{2}$ and $z_1 = \frac{\mu_1^{'} + \mu_2^{'}}{2}$. We may express this objective as a function of Q-functions which may be optimized numerically in the parameter space of $\beta_0, \beta_1, \beta_2$. For mixture of Gaussians distributions with uneven covariances, the resulting minimization procedure is an integral over different regions of Z for the conditional Gaussian distribution with highest probability.

\section{Noisy transformations with unequal covariances}
Given 

==> Sections/RemovedSections.tex <==
\section{ClassicDetectionremoved}
From detection theory we know the performance metric of a MAP detector of Gaussian hypotheses to be 
$d^2 = (\mu_0 + \beta_0 - (\mu_1 + \beta_1))^T \Sigma^{-1} (\mu_0 + \beta_0 - (\mu_1 + \beta_1)) = (\mu_0^{'} - \mu_1^{'})^T \Sigma^{-1} (\mu_0^{'} - \mu_1^{'})$. Subject to a total distortion constraint $(1-\tilde{p})\beta_0^T \beta_0 + \tilde{p}\beta_1^T \beta_1$, we have the following optimization problem:
\begin{equation}
\min d^2  \qquad s.t. \quad (1-\tilde{p})\beta_0^T \beta_0 + \tilde{p}\beta_1^T \beta_1 \le D
\end{equation}
By applying the Karuhn-Kush-Tucker (KKT)\cite{Boyd} conditions we have the following equations to solve for:
\begin{equation}
    \Sigma^{-1} (\mu_0 + \beta_0^* - (\mu_1 + \beta_1^*)) + \gamma^* (1-\tilde{p})\beta_0^* = 0
\end{equation}
\begin{equation}
    \Sigma^{-1} (\mu_0 + \beta_0^* - (\mu_1 + \beta_1^*)) + \gamma^* \tilde{p}\beta_1^* = 0
\end{equation}
\begin{equation}
    \gamma^* [(1-\tilde{p})\beta_0^{*T}\beta_0^* + \tilde{p}\beta_1^{*T}\beta_1^* -D] = 0
\end{equation}
Solving this set of equations for the variables $\beta_0^*, \beta_1^*, \gamma^*$ gives some insight into the structure of the optimal transformation vectors:
\begin{equation*}
    \beta_0^{*T}\beta_0^* = \ddfrac{\tilde{p}}{1-\tilde{p}} D, \qquad
    \beta_1^{*T}\beta_1^* = \ddfrac{1-\tilde{p}}{\tilde{p}} D
\end{equation*}
\begin{equation*}
    \beta_0^* = \tilde{p}[(1-2\tilde{p})I - \gamma^*\tilde{p}(1 - \tilde{p})\Sigma]^{-1}(\mu_0 - \mu_1)
\end{equation*}
\begin{equation*}
    \beta_1^* = \beta_0^* + \gamma^*(1 - \tilde{p})\Sigma \beta_0^* + (\mu_0 - \mu_1)
\end{equation*}

==> Sections/SibsonMI.tex <==
\section{Sibson Mutual Information as a metric}
%Reiterate problem statement
In this section we will use the Sibson mutual information as a privacy metric in the same optimization problem. The maximal information leakage may be intractable for numerical optimization, in which case the Sibson mutual information acts as a substitute metric. We know that \\
\begin{align*}
    I(Z \rightarrow C) = \log(\displaystyle\sum_c \displaystyle\max_z p_{C|Z})
    = I_\infty(Z;C)\\
    I_\alpha(Z;C) = \frac{\alpha}{\alpha - 1}\log(\displaystyle\sum_c (\displaystyle\sum_z p_{C|Z}^\alpha p_Z)^{\frac{1}{\alpha}})
\end{align*}
When we consider the initial 1D binary mixture of Gaussian case with affine transformations of the data, we have $p_C(0) = \tilde{p}$, $p_C(1) = 1 - \tilde{p}$, $p_{X|C=0} \sim \mathcal{N}(\mu_0, \sigma)$, $p_{X|C=1} \sim \mathcal{N}(\mu_1, \sigma)$. Under the transformation $Z = X + \beta_0 C + \beta_1 (1-C)$, we have $p(Z|C=0) \sim \mathcal{N}(\mu_0+\beta_0, \sigma)$, $p(Z|C=1) \sim \mathcal{N}(\mu_1+\beta_1, \sigma)$ as before. With this metric we have \\
\small
\begin{gather*}
    I_\alpha(Z;C) = \frac{\alpha}{\alpha - 1}\log(\displaystyle\int_z p_{C=0|Z}^\alpha p_Z)^{\frac{1}{\alpha}} + (\displaystyle\int_z p_{C=1|Z}^\alpha p_Z)^{\frac{1}{\alpha}} \\
    = \frac{\alpha}{\alpha - 1}\log[(\displaystyle\int_z (\ddfrac{p_{Z|C=0}\tilde{p}}{p_{Z|C=0}\tilde{p} + p_{Z|C=1}(1-\tilde{p})})^\alpha p_Z)^{\frac{1}{\alpha}} + \\
    (\displaystyle\int_z (\ddfrac{p_{Z|C=1}(1-\tilde{p})}{p_{Z|C=0}\tilde{p} + p_{Z|C=1}(1-\tilde{p})})^\alpha p_Z)^{\frac{1}{\alpha}}]
\end{gather*}
\normalsize
%change back font
%state the adversary performance as a theorem, characterize it in terms of the distortion budget, as part of an optimization
Examining the first term, we have $(\displaystyle\int_z (\ddfrac{p_{Z|C=0}\tilde{p}}{p_{Z|C=0}\tilde{p} + p_{Z|C=1}(1-\tilde{p})})^\alpha (\tilde{p}p_{Z|C=0} + (1-\tilde{p})p_{Z|C=1}))^{\frac{1}{\alpha}}$, so we wish to calculate $\mathbbm{E}_{Z|C=0}[(1 + \frac{1-\tilde{p}}{\tilde{p}}\ddfrac{p_{Z|C=1}}{p_{Z|C=0}})^{-\alpha}]$, and this doesn't admit an analytic solution, but we may bound it from above with $(\frac{1-\tilde{p}}{\tilde{p}}\ddfrac{p_{Z|C=1}}{p_{Z|C=0}})^{-\alpha}$. Applying the upper bound $(\frac{1-\tilde{p}}{\tilde{p}}\ddfrac{p_{Z|C=1}}{p_{Z|C=0}})^{-\alpha}$ to the first term yields
\small
\begin{gather*}
    \displaystyle\int_z (\frac{1-\tilde{p}}{\tilde{p}} \exp\ddfrac{\mu_0^{'2} - \mu_1^{'2}}{2\sigma^2} \exp \ddfrac{\mu'_1 - \mu'_0}{\sigma^2}z)^{-\alpha}\tilde{p}p_{Z|C=0} dz = \\
    \tilde{p}(\frac{1-\tilde{p}}{\tilde{p}} \exp\ddfrac{\mu_0^{'2} - \mu_1^{'2}}{2\sigma^2})^{-\alpha} \displaystyle\int_z \exp(-\alpha\ddfrac{\mu'_1 - \mu'_0}{\sigma^2}z) p_{Z|C=0} dz =\\
    \tilde{p} A^{-\alpha} \exp(\mu'_0(-\alpha B))\exp(\frac{\sigma^2 \alpha^2 B^2}{2})
\end{gather*}
\normalsize
%change back font
We can also upper bound the first term using a piece-wise function $g(z) = \min(1, (\frac{1-\tilde{p}}{\tilde{p}}\ddfrac{p_{Z|C=1}}{p_{Z|C=0}})^{-\alpha})$, which reaches 1 at $z_0 = (\log\frac{1 - \tilde{p}}{\tilde{p}} + \frac{\mu_0^{'2} - \mu_1^{'2}}{2\sigma^2})\ddfrac{\sigma^2}{\mu'_0 - \mu'_1}$. W.L.O.G. we may let $\mu'_1 < \mu'_0$, then
\small
\begin{gather*}
    \mathbbm{E}_{Z|C=0}[g(z)] = \\
    \displaystyle\int_{-\infty}^{z_0}A^{-\alpha}\exp(-\alpha Bz)p_{Z|C=0} dz + \displaystyle\int_{z_0}^{\infty}p_{Z|C=0} dz\\
    = (\ddfrac{1-\tilde{p}}{\tilde{p}}\exp(\ddfrac{\mu_0^{'2} - \mu_1^{'2}}{2\sigma^2}))^{-\alpha} \exp(\ddfrac{(\mu'_0 + \alpha(\mu'_0 - \mu'_1))^2 - \mu_0^{'2}}{2\sigma^2} \\
    [1-Q(\ddfrac{z_0 - (\mu'_0 + \alpha(\mu'_0 - \mu'_1))}{\sigma})] + Q(\ddfrac{z_0 - \mu'_0}{\sigma})
\end{gather*}
\normalsize
%change back font
where the Q function is commonly defined as\\
\begin{align*}
    Q(x) = 1 - \Phi(x) = 1 - \frac{1}{2}(1 + erf(\frac{x}{\sqrt{2}}))
\end{align*}
When applying the upper bound $(\frac{1-\tilde{p}}{\tilde{p}}\ddfrac{p_{Z|C=1}}{p_{Z|C=0}})^{-\alpha}$ and $(\frac{\tilde{p}}{1-\tilde{p}}\ddfrac{p_{Z|C=0}}{p_{Z|C=1}})^{-\alpha}$ to the terms in the loss function results in the following expression for the sibson mutual information:
\small
\begin{gather}
    I_{\alpha}(Z;C) = \frac{\alpha}{\alpha - 1}\log((h_0 + h_1)^{1/\alpha} + (h_2 + h_3)^{1/\alpha})\\
    = \frac{\alpha}{\alpha - 1} \log ([\tilde{p}(\frac{1-\tilde{p}}{\tilde{p}})^{-\alpha}\exp(\frac{(\alpha^2 + \alpha)}{2} d^2) + \\
    (1-\tilde{p})(\frac{1-\tilde{p}}{\tilde{p}})^{-\alpha}\exp(\frac{(\alpha^2 - \alpha)}{2} d^2)]^{1/\alpha} + \\
    [\tilde{p}(\frac{\tilde{p}}{1-\tilde{p}})^{-\alpha}\exp(\frac{(\alpha^2 + \alpha)}{2} d^2) + \\
    (1-\tilde{p})(\frac{\tilde{p}}{1-\tilde{p}})^{-\alpha}\exp(\frac{(\alpha^2 - \alpha)}{2} d^2)]^{1/\alpha})
\end{gather}
\normalsize
%change back font
where \begin{math}
d^2 = \frac{(\mu\prime_1 - \mu\prime_0)^2}{\sigma^2}
\end{math}. This bound indicates that the Sibson mutual information is a function of the distance between the transformed means when we consider affine transformations of Gaussian mixture data. Furthermore, it is monotonic in $d^2$, so minimization of the Sibson mutual information is equivalent to minimizing the adversary's performance for the considered data distribution and transformation.

